A Local Geometric Interpretation of Feature Extraction in Deep Feedforward Neural Networks

In this paper, we present a local geometric analysis to interpret how deep feedforward neural networks extract low-dimensional features from high-dimensional data. Our study shows that, in a local geometric region, the optimal weight in one layer of the neural network and the optimal feature generated by the previous layer comprise a low-rank approximation of a matrix that is determined by the Bayes action of this layer. This result holds (i) for analyzing both the output layer and the hidden layers of the neural network, and (ii) for neuron activation functions with non-vanishing gradients. We use two supervised learning problems to illustrate our results: neural network based maximum likelihood classification (i.e., softmax regression) and neural network based minimum mean square estimation. Experimental validation of these theoretical results will be conducted in our future work.

==> MainResult.tex <==







==> Score.tex <==
%!TEX root = ./DeepNeuralNet.tex

\section{Interpretation of Feature Generated in Neural Network}
In practice, hidden layers of the neural network may not generate $f^*(x)$ obtained in \eqref{optimal_feature}. If $t(x)=[t_1(x), \ldots, t_m(x)] \in \mathbb R^m$ is the input of the last hidden layer, then the feature $f(x)=g_{\mathbf{V}, c}(t(x))=[g(t(x)^{\operatorname{T}}v_1+c_1), \ldots, g(t(x)^{\operatorname{T}}v_m+c_m)]$, where $g(\cdot)$ is the activation function of the last hidden layer and $v_i=[v_{i, 1}, \ldots v_{i, m}] \in \mathbb R^m$ and $c_i$ are weights and bias, respectively that connects the $i$-th node of the last hidden layer and input $t(x)$. 

To quantify the closeness between any feature $f(x)$ and the optimal feature $f^*(x)$ obtained from \eqref{optimal_feature}, we consider 
\begin{align}
 \mathbb E_{X,Y \sim P_{X, Y}}\bigg[L\big(Y, h_{W, b}(f(x))\big)-L\big(Y, h_{W, b}(f^*(x))\big)\bigg].
\end{align}

To interpret the feature generated by neural network, we fix weight and bias $(W, b)$ of the output layer and consider the problem of designing weights $\mathbf{V}=[v_1, \ldots, v_k]$ and bias $c=[c_1, \ldots, c_k]$ that minimizes the score function $S(f^*, g_{\mathbf{V}, c}(t(x)))$ for any given input $t(x)$. We assume that $\mathbb E[t(X)]=0$.

Define matrices
\begin{align}
\mathbf{\Xi}_{t}=&[\sqrt{P_X(1)}t(1), \ldots, \sqrt{P_X(|\mathcal X|)}t(|\mathcal X|)], \\
J_1=&\text{diag}(g'(c_1), \ldots, g'(c_m)).
\end{align}
\begin{theorem}\label{theorem4}
If the conditions of Lemma \ref{lemma2} and $\mathbb E[t(X)]=0$, then for fixed weights and bias $(W, b)$ at the output layer
\begin{align}\label{ScoreApproximation}
& \mathbb E_{X,Y \sim P_{X, Y}}\bigg[L\big(Y, h_{W, b}(f(x))\big)-L\big(Y, h_{W, b}(f^*(x))\big)\bigg]\nonumber\\
=&\frac{1}{2}\|\mathbf{\Xi}_{\mathbf{W}}\mathbf{\Xi}_{f^*}-\mathbf{\Xi}_{\mathbf{V}}(\mathbf{\Xi}_{t})^{\operatorname{T}}\|_{F}^2+\frac{1}{2}\kappa_{W,b}(\mu_f)+o(\epsilon^2),
\end{align}
where $\mathbf{\Xi}_{\mathbf{V}}=\mathbf{\Xi}_{\mathbf{W}}\mathbf{J}_1\mathbf{V}$,  
\begin{align}
&\kappa_{W,b}(\mu_f) \nonumber\\
=&(2h_{0,\tilde b}(0)-2\mu_{a^*}+\mathbf{JW}\mu_f+d)^{\operatorname{T}}\mathbf{M}_L(\mathbf{JW}\mu_f+d)\nonumber\\
&-\eta_{W, d}(f^*),
\end{align}
and $\mu_f$ is given by
\begin{align}
\mu_f=g_{0,c}(0)+o(\epsilon).
\end{align}
\end{theorem}
\begin{proof}
See Appendix \ref{ptheorem4}
\end{proof}

Theorem \ref{theorem2} quantifies the closeness of the feature $f^*(x)$ and $g_{V, c}(t(x))$. To design the weights and bias $(V, c)$, we consider minimizing \eqref{ScoreApproximation} that can be separated into two optimization problems, given by
\begin{align}\label{weight_h}
\mathbf{\Xi}_{\mathbf{V}^*}=\arg \min_{\mathbf{\Xi}_{\mathbf{V}}} \frac{1}{2}\|\mathbf{\Xi}_{\mathbf{W}}\mathbf{\Xi}_{f^*}-\mathbf{\Xi}_V\mathbf{\Xi}_t^{\operatorname{T}}\|_{F}^2,
\end{align}
\begin{align}\label{bias_h}
\mu_f^*=\arg\min_{\mu_f} \kappa_{\mathbf{W},b}(\mu_f).
\end{align}

\begin{theorem}\label{theorem5}
An optimal solution $\tilde \Xi^{V^*}$ to \eqref{weight_h} is 
\begin{align}\label{optimal_weight_h}
\mathbf{\Xi}_{\mathbf{V}^*}=\mathbf{\Xi}_{\mathbf{W}}\mathbf{\Xi}_{f^*} \mathbf{\Xi}_t (\mathbf{\Xi}_t^{\operatorname{T}}\mathbf{\Xi}_t)^{-1},
\end{align}
the corresponding weight matrix $V$ is expressed as 
\begin{align}\label{optimal_weight_h_1}
V=\mathbf{J}_1^{-1}\mathbf{\Xi}_{f^*} \mathbf{\Xi}_t (\mathbf{\Xi}_t^{\operatorname{T}}\mathbf{\Xi}_t)^{-1},
\end{align}
the optimal solution $\mu_f^*$ to \eqref{bias_h} is given by
\begin{align}\label{optimal_bias_h}
\mu_f^*=\mu_{f^*},
\end{align}
and the corresponding bias vector $c$ is given by 
\begin{align}
c=g^{-1}(\mu_{f^*})+o(\epsilon).
\end{align}
\end{theorem}

Theorem \ref{theorem5} illustrates that the optimal weight matrix $V$ is obtained by projecting optimal feature $f^*(x)$ onto the subspace of feature functions spanned by $t(x)$. This argument can be generalized to the weights of any intermediate layer of a deep neural network.  

In the learning process of a deep neural network, the backpropagation algorithm alternatively chooses weight matrix $\mathbf{W}$ and $\mathbf{V}$. This is equivalent as alternately executing \eqref{optimal_weight_1} and \eqref{optimal_weight_h_1}.

